ACQUIRED: A Dataset for Answering Counterfactual Questions In Real-Life Videos

Multimodal counterfactual reasoning is a vital yet challenging ability for AI systems. It involves predicting the outcomes of hypothetical circumstances based on vision and language inputs, which enables AI models to learn from failures and explore hypothetical scenarios. Despite its importance, there are only a few datasets targeting the counterfactual reasoning abilities of multimodal models. Among them, they only cover reasoning over synthetic environments or specific types of events (e.g. traffic collisions), making them hard to reliably benchmark the model generalization ability in diverse real-world scenarios and reasoning dimensions. To overcome these limitations, we develop a video question answering dataset, ACQUIRED: it consists of 3.9K annotated videos, encompassing a wide range of event types and incorporating both first and third-person viewpoints, which ensures a focus on real-world diversity. In addition, each video is annotated with questions that span three distinct dimensions of reasoning, including physical, social, and temporal, which can comprehensively evaluate the model counterfactual abilities along multiple aspects. We benchmark our dataset against several state-of-the-art language-only and multimodal models and experimental results demonstrate a significant performance gap (>13%) between models and humans. The findings suggest that multimodal counterfactual reasoning remains an open challenge and ACQUIRED is a comprehensive and reliable benchmark for inspiring future research in this direction.

==> figs/model_archis.tex <==
\begin{figure*}[t!]
\centering

\begin{subfigure}[b]{.35\textwidth}
  \centering
  \includegraphics[width=.98\textwidth]{figs/imgs/non_context_model.pdf}
  \caption{Non-Contextualized Model}
  \label{fig:non_context_model}
\end{subfigure}%
\begin{subfigure}[b]{.63\textwidth}
  \centering
  \includegraphics[width=.98\textwidth]{figs/imgs/context_model.pdf}
  \caption{Contextualized Model}
  \label{fig:context_model}
\end{subfigure}
\vspace{-.6em}
\caption{ \footnotesize
\textbf{Model architectures:} 
\textbf{(a) Non-contextualized model:} The model only considers a pair of given text segments.
\textbf{(b) Contextualized model:} The model takes the whole instruction paragraphs (\ie contexts) and wrap each text segment with our special tokens (\texttt{<a>}), where each segment representation is obtained by taking an average over its token representations. The \textit{ordered} concatenated segment representations will then be fed into an MLP to make the final predictions. 
}
\label{fig:model_archis}
\vspace{-.3em}
\end{figure*}

==> figs/multi_template.tex <==
\begin{figure*}[t!]

\begin{subtable}{\textwidth}
\centering
\centering
    \includegraphics[width=.95\columnwidth]{figs/imgs/placeholder.png}
\caption{\footnotesize xxx}
\label{fig:ui_instr}
\end{subtable}

\begin{subtable}{\textwidth}
\centering
\centering
    \includegraphics[width=.95\columnwidth]{figs/imgs/placeholder.png}
\caption{\footnotesize yyy}
\label{fig:ui_ui}
\end{subtable}

\caption{ \footnotesize

}
\label{fig:ui}
\end{figure*}

==> figs/overall_radar_charts_nouns.tex <==
\begin{figure}
    \centering
    \includegraphics[width=.9\columnwidth]{figs/imgs/top-k-nouns-overall.pdf}
    \vspace{-.5em}
    \caption{
        \textbf{Top-40 frequent \underline{nouns}} in the dataset.
    }
    \label{fig:overall_radar_nouns}
\end{figure}

==> figs/terminologies.tex <==
\definecolor{LightBlue}{rgb}{0.78,1,1}
\definecolor{LightYellow}{rgb}{1,1,0.68}
\definecolor{LightGreen}{rgb}{0.78,1,0.78}

\begin{figure*}[t!]
\centering
    \includegraphics[width=.99\textwidth]{figs/imgs/terminology_srl.pdf}
    \vspace{-.3em}
    \caption{
    \footnotesize
    \textbf{Terminologies:}
    \textbf{(Left)} shows a few exemplar\colorbox{LightYellow}{actionables}with their associated\colorbox{LightBlue}{preconditions}and\colorbox{LightGreen}{postconditions}.
    Notice that an actionable can have multiple pre- or postconditions and they can span across different instruction steps
    (for simplicity we do not show an exhausted set of text segments, and the actual instruction contexts are much longer).
    % , \ie in the actual dataset there might be more.
    \textbf{(Right)} SRL is used to postulate the text segments (actionables and conditions).
    We show a sample SRL extraction corresponding to one of the dependency linkages on the left.
    The SRL~\texttt{ARG} labels also provide useful information for designing our heuristics (\secref{sec:data_heus}).
    % When multiple argument patterns exist for the same verb, we determine the segments by maximizing both the number of plausible segments within a sentence and the number of \texttt{ARG}s in each segment.
    % \telin{Say that actual article is much longer.}
    }
    \label{fig:term}
    % \vspace{-1.em}
\end{figure*}

==> tables/error_analysis.tex <==
\newcolumntype{G}{>{\centering\arraybackslash}m{.135\columnwidth}}
\newcolumntype{H}{>{\arraybackslash}m{.52\columnwidth}}
\newcolumntype{J}{>{\arraybackslash}m{.19\columnwidth}}

\begin{table}[t!]
\centering
\small
% \scalebox{.88}{
    \renewcommand{\arraystretch}{0.5} % Tighter
    \begin{tabular}{G|H|J}
    \toprule
    \multicolumn{1}{c|}{\textbf{Type}} & \multicolumn{1}{c|}{\textbf{Example}} & \multicolumn{1}{c}{\textbf{Description}} \\
    \midrule % \\[-1.1em]

    Heus. Overfit
    & \scalebox{.7}{\raisebox{.\height}{\includegraphics[width=.75\columnwidth]{figs/imgs/error_example_heus_overfit.pdf}}} & Overfits on entity trace heuristic. \\

    \midrule % \\[-1.1em]
    
    Lacking Causal Reason
    & \scalebox{.7}{\raisebox{.\height}{\includegraphics[width=.78\columnwidth]{figs/imgs/error_example_causality.pdf}}} & Knowledge-enhanced causal reasoning can be helpful. \\
    
    \bottomrule
    \end{tabular}
% }
\vspace{-.8em}
\caption{
\footnotesize
\textbf{Exemplar model errors.} The second row are from distant segments not link-able even via the keyword heuristic.
% The color schemes are the same as~\figref{fig:term}.
}
\label{tab:error_sample_table}
% \vspace{-1.em}
\end{table}

==> tables/other_forward_videoqa_results.tex <==
\begin{table}[t!]
\centering
\small\addtolength{\tabcolsep}{-2.4pt}
\scalebox{.95}{
    \begin{tabular}{c|cccc}
    \toprule
    \textbf{Model} & TVQA & How2QA & Dataset-C & Dataset-D \\
    \midrule 
    VIOLET         & 00.00     &  00.00    & 00.00     & 00.00  \\
    VALOR          & 00.00     &  00.00    & 00.00     & 00.00  \\
    VL-Adapter     & 76.6     &  73.9    & 00.00     & 00.00  \\
    \bottomrule
    \end{tabular}
}
\vspace{-.6em}
\caption{
\footnotesize
\zd{only VL-Adapter tests on mcq datasets (others are open-ended qa datasets) and their VL-Adapter model is based on BART-base. may remove this comparison?}
\textbf{Performance on factual reasoning video QA datasets.} We report the performance of the models used in this work on existing non-counterfactual video QA, as a reference.
}
\label{tab:factual_datasets_results}
\end{table}

==> text/task.tex <==
\section{Terminologies and Problem Definition}
...
